BigColor: Colorization using a Generative Color Prior for Natural Images

For realistic and vivid colorization, generative priors have recently been exploited. However, such generative priors often fail for in-the-wild complex images due to their limited representation space. In this paper, we propose BigColor, a novel colorization approach that provides vivid colorization for diverse in-the-wild images with complex structures. While previous generative priors are trained to synthesize both image structures and colors, we learn a generative color prior to focus on color synthesis given the spatial structure of an image. In this way, we reduce the burden of synthesizing image structures from the generative prior and expand its representation space to cover diverse images. To this end, we propose a BigGAN-inspired encoder-generator network that uses a spatial feature map instead of a spatially-flattened BigGAN latent code, resulting in an enlarged representation space. Our method enables robust colorization for diverse inputs in a single forward pass, supports arbitrary input resolutions, and provides multi-modal colorization results. We demonstrate that BigColor significantly outperforms existing methods especially on in-the-wild images with complex structures.

==> tables/tbl_ablation_fdim.tex <==
\begin{table}[t]
\begin{center}
\caption{
\sh{check:}
The spatial resolution of the input-image feature $f$ plays an important role for maintaining a balance for the tradeoff between keeping the spatial structure of the input and providing the degree of freedom for the color synthesis. $16 \times 16$ provides the best colorfulness score. % Colorfulness scores gradually decrease from the 8 x 8 feature resolution to the high resolution due to the reduction of generative color prior
}
\setlength{\tabcolsep}{1.2em}
\begin{tabular}{c|*{5}{c}}
\hline
 & Latent Z & 8 x 8 & 16 x 16 & 32 x 32 & 64 x 64 \\
\hline\hline
FID~\cite{FID}                 & 19.230 & 13.103 & 5.714  & {\bf 5.384}  & 6.120 \\
Colorful~\cite{Colorfulness}   & 31.683 & 39.547 & {\bf 33.706} & 33.370 & 30.497 \\
\hline
\end{tabular}
%\vspace{+0.3cm}

\label{table:ablation_fdim}
\end{center}
\end{table}

==> texts/g_others.tex <==
\begin{abstract}
The abstract should summarize the contents of the paper. LNCS guidelines
indicate it should be at least 70 and at most 150 words. It should be set in 9-point
font size and should be inset 1.0~cm from the right and left margins.
\dots
\keywords{We would like to encourage you to list your keywords within
the abstract section}
\end{abstract}


\section{Initial Submission}

\subsection{Language}

All manuscripts must be in English.

\subsection{Paper length}
Papers submitted for review should be complete. 
The length should match that intended for final publication. 
Papers accepted for the conference will be allocated 14 pages (plus references) in the proceedings. 
Note that the allocated 14 pages do not include the references. The reason for this policy
is that we do not want authors to omit references for sake of space limitations.

Papers with more than 14 pages (excluding references) will be rejected without review.
This includes papers where the margins and
formatting are deemed to have been significantly altered from those
laid down by this style guide. Do not use the TIMES, or any other font than the default. The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts. The reviewing process cannot determine the suitability of the paper for presentation in 14 pages if it is reviewed in 16.

\subsection{Paper ID}

It is imperative that the paper ID is mentioned on each page of the manuscript.
The paper ID is a number automatically assigned to your submission when 
registering your paper submission on the submission site.

%\subsection{Line numbering}

All lines should be numbered in the initial submission, as in this example document. This makes reviewing more efficient, because reviewers can refer to a line on a page. Line numbering is removed in the camera-ready.


\subsection{Mathematics}

Please number all of your sections and displayed equations.  Again,
this makes reviewing more efficient, because reviewers can refer to a
line on a page.  Also, it is important for readers to be able to refer
to any particular equation.  Just because you didn't refer to it in
the text doesn't mean some future reader might not need to refer to
it.  It is cumbersome to have to use circumlocutions like ``the
equation second from the top of page 3 column 1''.  (Note that the
line numbering will not be present in the final copy, so is not an
alternative to equation numbers).  Some authors might benefit from
reading Mermin's description of how to write mathematics:
\url{www.pamitc.org/documents/mermin.pdf}.


\section{Policies}
\subsection{Review Process}
By submitting a paper to ECCV, the authors agree to the review process and understand that papers are processed by the Toronto system to match each manuscript to the best possible chairs and reviewers.
\subsection{Confidentiality}
The review process of ECCV is confidential. Reviewers are volunteers not part of the ECCV organisation and their efforts are greatly appreciated. The standard practice of keeping all information confidential during the review is part of the standard communication to all reviewers. Misuse of confidential information is a severe professional failure and  appropriate measures will be taken when brought to the attention of ECCV organizers. It should be noted, however, that the organisation of ECCV is not and cannot be held responsible for the consequences when reviewers break confidentiality.

Accepted papers will be published by Springer (with appropriate copyrights) electronically up to three weeks prior to the main conference. Please make sure to discuss this issue with your legal advisors as it pertains to public disclosure of the contents of the papers submitted.
\subsection{Dual and Double Submissions}
By submitting a manuscript to ECCV 2020, authors acknowledge that it has not been previously published or accepted for publication in substantially similar form in any peer-reviewed venue including journal, conference, or workshop. Furthermore, no paper substantially similar in content has been or will be submitted to a journal, another conference or workshop during the review period (March 05, 2020 – July 3, 2020). The authors also attest that they did not submit substantially similar submissions to ECCV 2020. Violation of any of these conditions will lead to rejection and the violation will be reported to the other venue or journal, which will typically lead to rejection there as well. 

The goals of the dual submission policy are (i) to have exciting new work be published for the first time at ECCV 2020, and (ii) to avoid duplicating the efforts of the reviewers.
Therefore, all papers under review are checked for dual submissions and this is not allowed, independent of the page size of submissions. 

For already published papers, our policy is based upon the following particular definition of ``publication''. A publication, for the purposes of the dual submission policy, is defined to be a written work longer than four pages that was submitted for review by peers for either acceptance or rejection, and, after review, was accepted. In particular, this definition of publication does not depend upon whether such an accepted written work appears in a formal proceedings or whether the organizers declare that such work ``counts as a publication''. 

An arXiv.org paper does not count as a publication because it was not peer-reviewed for acceptance. The same is true for university technical reports. However, this definition of publication does include peer-reviewed workshop papers, even if they do not appear in a proceedings, if their length is more than 4 pages including citations. Given this definition, any submission to ECCV 2020 should not have substantial overlap with prior publications or other concurrent submissions. As a rule of thumb, the ECCV 2020 submission should contain no more than 20 percent of material from previous publications. 

\subsection{Requirements for publication}
Publication of the paper in the ECCV 2020 proceedings of Springer requires that at least one of the authors registers for the conference and present the paper there. It also requires that a camera-ready version that satisfies all formatting requirements is submitted before the camera-ready deadline. 
\subsection{Double blind review}
\label{sec:blind}
ECCV reviewing is double blind, in that authors do not know the names of the area chair/reviewers of their papers, and the area chairs/reviewers cannot, beyond reasonable doubt, infer the names of the authors from the submission and the additional material. Avoid providing links to websites that identify the authors. Violation of any of these guidelines may lead to rejection without review. If you need to cite a different paper of yours that is being submitted concurrently to ECCV, the authors should (1) cite these papers, (2) argue in the body of your paper why your ECCV paper is non trivially different from these concurrent submissions, and (3) include anonymized versions of those papers in the supplemental material.

Many authors misunderstand the concept of anonymizing for blind
review. Blind review does not mean that one must remove
citations to one's own work. In fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
technical reports).

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith, it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an excellent paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L. and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same
time, which covers similar or overlapping material, you may need
to refer to that submission in order to explain the differences,
just as you would if you had previously published related work. In
such cases, include the anonymized parallel
submission~\cite{Authors14} as additional material and cite it as
\begin{quote}
1. Authors. ``The frobnicatable foo filter'', BMVC 2014 Submission
ID 324, Supplied as additional material {\tt bmvc14.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more
details can be found elsewhere, and refer them to a technical
report.  For conference submissions, the paper must stand on its
own, and not {\em require} the reviewer to go to a techreport for
further details.  Thus, you may say in the body of the paper
``further details may be found in~\cite{Authors14b}''.  Then
submit the techreport as additional material. Again, you may not
assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the ECCV audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B. \\

For sake of anonymity, it's recommended to omit acknowledgements
in your review copy. They can be added later when you prepare the final copy.

\section{Manuscript Preparation}

This is an edited version of Springer LNCS instructions adapted
for ECCV 2020 first paper submission.
You are strongly encouraged to use \LaTeX2$_\varepsilon$ for the
preparation of your
camera-ready manuscript together with the corresponding Springer
class file \verb+llncs.cls+.

We would like to stress that the class/style files and the template
should not be manipulated and that the guidelines regarding font sizes
and format should be adhered to. This is to ensure that the end product
is as homogeneous as possible.

\subsection{Printing Area}
The printing area is $122  \; \mbox{mm} \times 193 \;
\mbox{mm}$.
The text should be justified to occupy the full line width,
so that the right margin is not ragged, with words hyphenated as
appropriate. Please fill pages so that the length of the text
is no less than 180~mm.

\subsection{Layout, Typeface, Font Sizes, and Numbering}
Use 10-point type for the name(s) of the author(s) and 9-point type for
the address(es) and the abstract. For the main text, please use 10-point
type and single-line spacing.
We recommend using Computer Modern Roman (CM) fonts, which is the default font in this template.
Italic type may be used to emphasize words in running text. Bold
type and underlining should be avoided.
With these sizes, the interline distance should be set so that some 45
lines occur on a full-text page.

\subsubsection{Headings.}

Headings should be capitalized
(i.e., nouns, verbs, and all other words
except articles, prepositions, and conjunctions should be set with an
initial capital) and should,
with the exception of the title, be aligned to the left.
Words joined by a hyphen are subject to a special rule. If the first
word can stand alone, the second word should be capitalized.
The font sizes
are given in Table~\ref{table:headings}.
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Font sizes of headings. Table captions should always be
positioned {\it above} the tables. The final sentence of a table
caption should end without a full stop}
\label{table:headings}
\begin{tabular}{lll}
\hline\noalign{\smallskip}
Heading level & Example & Font size and style\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Title (centered)  & {\Large \bf Lecture Notes \dots} & 14 point, bold\\
1st-level heading & {\large \bf 1 Introduction} & 12 point, bold\\
2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold
\\
4th-level heading & {\it Remark.} Text follows \dots & 10 point,
italic\\
\hline
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

Here are some examples of headings: ``Criteria to Disprove Context-Freeness of
Collage Languages'', ``On Correcting the Intrusion of Tracing
Non-deterministic Programs by Software'', ``A User-Friendly and
Extendable Data Distribution System'', ``Multi-flip Networks:
Parallelizing GenSAT'', ``Self-determinations of Man''.

\subsubsection{Lemmas, Propositions, and Theorems.}

The numbers accorded to lemmas, propositions, and theorems etc. should
appear in consecutive order, starting with the number 1, and not, for
example, with the number 11.

\subsection{Figures and Photographs}
\label{sect:figures}

Please produce your figures electronically and integrate
them into your text file. For \LaTeX\ users we recommend using package
\verb+graphicx+ or the style files \verb+psfig+ or \verb+epsf+.

Check that in line drawings, lines are not
interrupted and have constant width. Grids and details within the
figures must be clearly readable and may not be written one on top of
the other. Line drawings should have a resolution of at least 800 dpi
(preferably 1200 dpi).
For digital halftones 300 dpi is usually sufficient.
The lettering in figures should have a height of 2~mm (10-point type).
Figures should be scaled up or down accordingly.
Please do not use any absolute coordinates in figures.

Figures should be numbered and should have a caption which should
always be positioned {\it under} the figures, in contrast to the caption
belonging to a table, which should always appear {\it above} the table.
Please center the captions between the margins and set them in
9-point type
(Fig.~\ref{fig:example} shows an example).
The distance between text and figure should be about 8~mm, the
distance between figure and caption about 5~mm.
\begin{figure}
\centering
\includegraphics[height=6.5cm]{eijkel2}
\caption{One kernel at $x_s$ ({\it dotted kernel}) or two kernels at
$x_i$ and $x_j$ ({\it left and right}) lead to the same summed estimate
at $x_s$. This shows a figure consisting of different types of
lines. Elements of the figure described in the caption should be set in
italics,
in parentheses, as shown in this sample caption. The last
sentence of a figure caption should generally end without a full stop}
\label{fig:example}
\end{figure}

If possible (e.g. if you use \LaTeX) please define figures as floating
objects. \LaTeX\ users, please avoid using the location
parameter ``h'' for ``here''. If you have to insert a pagebreak before a
figure, please ensure that the previous page is completely filled.


\subsection{Formulas}

Displayed equations or formulas are centered and set on a separate
line (with an extra line or halfline space above and below). Displayed
expressions should be numbered for reference. The numbers should be
consecutive within the contribution,
with numbers enclosed in parentheses and set on the right margin.
For example,
\begin{align}
  \psi (u) & = \int_{0}^{T} \left[\frac{1}{2}
  \left(\Lambda_{0}^{-1} u,u\right) + N^{\ast} (-u)\right] dt \; \\
& = 0 ?
\end{align}

Please punctuate a displayed equation in the same way as ordinary
text but with a small space before the end punctuation.

\subsection{Footnotes}

The superscript numeral used to refer to a footnote appears in the text
either directly after the word to be discussed or, in relation to a
phrase or a sentence, following the punctuation sign (comma,
semicolon, or full stop). Footnotes should appear at the bottom of
the
normal text area, with a line of about 2~cm in \TeX\ and about 5~cm in
Word set
immediately above them.\footnote{The footnote numeral is set flush left
and the text follows with the usual word spacing. Second and subsequent
lines are indented. Footnotes should end with a full stop.}


\subsection{Program Code}

Program listings or program commands in the text are normally set in
typewriter font, e.g., CMTT10 or Courier.

\noindent
{\it Example of a Computer Program}
\begin{verbatim}
program Inflation (Output)
  {Assuming annual inflation rates of 7%, 8%, and 10%,...
   years};
   const
     MaxYears = 10;
   var
     Year: 0..MaxYears;
     Factor1, Factor2, Factor3: Real;
   begin
     Year := 0;
     Factor1 := 1.0; Factor2 := 1.0; Factor3 := 1.0;
     WriteLn('Year  7% 8% 10%'); WriteLn;
     repeat
       Year := Year + 1;
       Factor1 := Factor1 * 1.07;
       Factor2 := Factor2 * 1.08;
       Factor3 := Factor3 * 1.10;
       WriteLn(Year:5,Factor1:7:3,Factor2:7:3,Factor3:7:3)
     until Year = MaxYears
end.
\end{verbatim}
%
\noindent
{\small (Example from Jensen K., Wirth N. (1991) Pascal user manual and
report. Springer, New York)}



\subsection{Citations}

The list of references is headed ``References" and is not assigned a
number
in the decimal system of headings. The list should be set in small print
and placed at the end of your contribution, in front of the appendix,
if one exists.
Please do not insert a pagebreak before the list of references if the
page is not completely filled.
An example is given at the
end of this information sheet. For citations in the text please use
square brackets and consecutive numbers: \cite{Alpher02},
\cite{Alpher03}, \cite{Alpher04} \dots

\section{Submitting a Camera-Ready for an Accepted Paper}
\subsection{Converting Initial Submission to Camera-Ready}
To convert a submission file into a camera-ready for an accepted paper:
\begin{enumerate}
    \item  First comment out \begin{verbatim}
        \usepackage{ruler}
    \end{verbatim} and the line that follows it.
    \item  The anonymous title part should be removed or commented out, and a proper author block should be inserted, for which a skeleton is provided in a commented-out version. These are marked in the source file as \begin{verbatim}
        % INITIAL SUBMISSION 
    \end{verbatim} and \begin{verbatim}
        % CAMERA READY SUBMISSION 
    \end{verbatim}
    \item Please write out author names in full in the paper, i.e. full given and family names. If any authors have names that can be parsed into FirstName LastName in multiple ways, please include the correct parsing in a comment to the editors, below the \begin{verbatim}\author{}\end{verbatim} field.
    \item Make sure you have inserted the proper Acknowledgments.
  \end{enumerate}  
 
\subsection{Preparing the Submission Package}
We need all the source files (LaTeX files, style files, special fonts, figures, bib-files) that are required to compile papers, as well as the camera ready PDF. For each paper, one ZIP-file called XXXX.ZIP (where XXXX is the zero-padded, four-digit paper ID) has to be prepared and submitted via the ECCV 2020 Submission Website, using the password you received with your initial registration on that site. The size of the ZIP-file may not exceed the limit of 60 MByte. The ZIP-file has to contain the following:
  \begin{enumerate}
 \item  All source files, e.g. LaTeX2e files for the text, PS/EPS or PDF/JPG files for all figures.
 \item PDF file named ``XXXX.pdf" that has been produced by the submitted source, where XXXX is the four-digit paper ID (zero-padded if necessary). For example, if your paper ID is 24, the filename must be 0024.pdf. This PDF will be used as a reference and has to exactly match the output of the compilation.
 \item PDF file named ``XXXX-copyright.PDF": a scanned version of the signed copyright form (see ECCV 2020 Website, Camera Ready Guidelines for the correct form to use). 
 \item If you wish to provide supplementary material, the file name must be in the form XXXX-supp.pdf or XXXX-supp.zip, where XXXX is the zero-padded, four-digit paper ID as used in the previous step. Upload your supplemental file on the ``File Upload" page as a single PDF or ZIP file of 100 MB in size or less. Only PDF and ZIP files are allowed for supplementary material. You can put anything in this file – movies, code, additional results, accompanying technical reports–anything that may make your paper more useful to readers.  If your supplementary material includes video or image data, you are advised to use common codecs and file formats.  This will make the material viewable by the largest number of readers (a desirable outcome). ECCV encourages authors to submit videos using an MP4 codec such as DivX contained in an AVI. Also, please submit a README text file with each video specifying the exact codec used and a URL where the codec can be downloaded. Authors should refer to the contents of the supplementary material appropriately in the paper.
 \end{enumerate}

Check that the upload of your file (or files) was successful either by matching the file length to that on your computer, or by using the download options that will appear after you have uploaded. Please ensure that you upload the correct camera-ready PDF–renamed to XXXX.pdf as described in the previous step as your camera-ready submission. Every year there is at least one author who accidentally submits the wrong PDF as their camera-ready submission.

Further considerations for preparing the camera-ready package:
  \begin{enumerate}
    \item Make sure to include any further style files and fonts you may have used.
    \item References are to be supplied as BBL files to avoid omission of data while conversion from BIB to BBL.
    \item Please do not send any older versions of papers. There should be one set of source files and one XXXX.pdf file per paper. Our typesetters require the author-created pdfs in order to check the proper representation of symbols, figures, etc.
    \item  Please remove unnecessary files (such as eijkel2.pdf and eijkel2.eps) from the source folder. 
    \item  You may use sub-directories.
    \item  Make sure to use relative paths for referencing files.
    \item  Make sure the source you submit compiles.
\end{enumerate}

Springer is the first publisher to implement the ORCID identifier for proceedings, ultimately providing authors with a digital identifier that distinguishes them from every other researcher. ORCID (Open Researcher and Contributor ID) hosts a registry of unique researcher identifiers and a transparent method of linking research activities to these identifiers. This is achieved through embedding ORCID identifiers in key workflows, such as research profile maintenance, manuscript submissions, grant applications and patent applications.
\subsection{Most Frequently Encountered Issues}
Please kindly use the checklist below to deal with some of the most frequently encountered issues in ECCV submissions.

{\bf FILES:}
\begin{itemize}
    \item My submission package contains ONE compiled pdf file for the camera-ready version to go on Springerlink.
\item I have ensured that the submission package has all the additional files necessary for compiling the pdf on a standard LaTeX distribution.
\item I have used the correct copyright form (with editor names pre-printed), and a signed pdf is included in the zip file with the correct file name.
\end{itemize}

{\bf CONTENT:}
\begin{itemize}
\item I have removed all \verb \vspace  and \verb \hspace  commands from my paper.
\item I have not used \verb \thanks  or \verb \footnote  commands and symbols for corresponding authors in the title (which is processed with scripts) and (optionally) used an Acknowledgement section for all the acknowledgments, at the end of the paper.
\item I have not used \verb \cite  command in the abstract.
\item I have read the Springer author guidelines, and complied with them, including the point on providing full information on editors and publishers for each reference in the paper (Author Guidelines – Section 2.8).
\item I have entered a correct \verb \titlerunning{}  command and selected a meaningful short name for the paper.
\item I have entered \verb \index{Lastname,Firstname}  commands for names that are longer than two words.
\item I have used the same name spelling in all my papers accepted to ECCV and ECCV Workshops.
\item I have inserted the ORCID identifiers of the authors in the paper header (see http://bit.ly/2H5xBpN for more information).
\item I have not decreased the font size of any part of the paper (except tables) to fit into 14 pages, I understand Springer editors will remove such commands.
\end{itemize}
{\bf SUBMISSION:}
\begin{itemize}
\item All author names, titles, and contact author information are correctly entered in the submission site.
\item The corresponding author e-mail is given.
\item At least one author has registered by the camera ready deadline.
\end{itemize}

==> texts/z_supple.tex <==
\setcounter{section}{0}
\renewcommand\thesection{\Alph{section}}

\begin{center}
{\Large \bf Supplemental Document}
\end{center}

\section{Qualitative and Quantitative Comparison}
For qualitative comparison to previous methods, we estimated the color results using official implementations for each method except for ToVivid~\cite{TowardVivid} due to the absence of released code.
Instead of reproducing the method of ToVivid and directly estimating the color image from a grayscale image, we requested and received the colorization results of ToVivid~\cite{TowardVivid} from the author.
For the case of DeOldify, which supports {\it stable} and {\it artistic} versions, we chose the stable version showing better performance on the ImageNet~\cite{ImageNet} validation set.

For clear perceptual comparison, all estimated images require identical resolution.
While the CNN-based colorization methods~\cite{CIC,ChromaGAN,InstColor,Deoldify} used in the comparison free from constraints to image resolution and aspect ratio, Coltran~\cite{ColTran} and ToVivid~\cite{TowardVivid} only enable producing the fixed size output with $256 \times 256$ spatial.
To overcome the constraint, ToVivid adopted a trick that resizes the grayscale image to $256 \times 256$ resolution ignoring the aspect ratio.
However, ColTran was vulnerable to the resizing trick due to their downsampling scheme of $64 \times 64$ low resolution.
As a result, we used the $256 \times 256$ resolution for all qualitative comparisons to compare in a situation where all methods are operable.

In this supplemental document, we provide more qualitative and quantitative comparisons. Specifically, qualitative comparison for general image in ImageNet1K validation set shown in \Figs{\ref{fig:sup_cmp1}~\ref{fig:sup_cmp2}~\ref{fig:sup_cmp3}}, qualitative and quantitative comparison for complex images shown in \Fig{\ref{fig:sup_cplx1}} and \Tbl{\ref{table:sup_cplx_fid_color}}.


\section{Qualitative Examples}
We provide more qualitative examples of BigColor, consisting of multi-modal solutions with random code z shown in \Fig{\ref{fig:sup_multimodal}}, color results before and after Lab fusion shown in \Fig{\ref{fig:sup_rgb_lab}}, uncureated colorization results shown in \Figs{\ref{fig:sub_uncurate3}~\ref{fig:sub_uncurate3}}, and examples with limitations shown in \Fig{\ref{fig:sup_limitation}}.


\section{Architecture Details}
We attempted to find an optimal encoder architecture considering the type of activation functions, sequence of the modules, various normalization schemes.
After thorough architecture search, we amount to the current encoder architecture, resulting in the architecture analogous to the BigGAN generator. 
The non-local layer, an crucial component of the original BigGAN generator, is excluded in our encoder due to no performance improvement experimentally.
Drop-out module slightly improve the qualitative performance.

For the generator, we adopt fine layers of BigGAN initialized with pretrained parameters using ImageNet1K training set with $256 \times 256$ resolution. 
The random-sampled $z$ has a dimension of $68 \times 1$, which is different from the original dimension of 119 x 1, as we only use part of the BigGAN generator.
This one dimensional vector is divided into four parts of $17 \times 1$ resolution, concatenated with class code $c$ and amount to $145 \times 1$ dimension.
See \Fig\ref{fig:sup_architecture_detail}.

\section{Color Enhancement Augmentation}

\kkw{Describe details}


\section{User Study Details}
As shown in \Fig\ref{fig:sup_userstudy_gui}, we use a trap image for all test samples in order to filter the insincere participants in Amazon Mechanical Turk (AMT). The trap image is identical to the grayscale reference image. We excluded the subjects who select the trap image as the best colorization result at least one of the 100 test samples. In this way, we found 167 unfaithful ones from 200 total subjects, amounting to selected 33 participants. To select the 100 grayscale images for the test, we randomly sampled color images from ImageNet1K validation set, applied the grayscale transformation, and estimated the color for gray inputs using target colorization methods. To avoid potential bias from the method order, we shuffled the sequence of color image results for all tests.

%%%%%%%%%%%%%%% TEXT END %%%%%%%%%%%%%%%
\input{figures_supple/cmp}
\input{figures_supple/cplx}
\input{tables_supple/tbl_cplx_fid_color}

\input{figures_supple/multimodal}
\input{figures_supple/rgb_lab}
\input{figures_supple/uncurate}
\input{figures_supple/limitation}

\input{figures_supple/architecture_detail}

% Color Enhancement Augmentation

\input{figures_supple/userstudy_gui}
\input{tables_supple/tbl_userstudy}

==> texts/z_supple_kkang.tex <==
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}

% \renewcommand\thesection{\Alph{section}}
\renewcommand\thefigure{S\arabic{figure}}
\renewcommand\thetable{S\arabic{table}}

\begin{center}
{\Large \bf BigColor: Colorization using \\ a Generative Color Prior for Natural Images\\ \footnotesize ~ \\\Large-- Supplemental Document --}
\end{center}

In this Supplemental Document, we present additional details, analysis, and results. Specifically, we provide:
\begin{itemize}
    \item Details on the network architecture,
    \item User study details,
    \item Additional discussion on the color enhancement augmentation,
    \item Additional examples of the luminance replacement,
    \item Qualitative and quantitative comparisons,
    \item Additional uncurated examples,
    \item Additional examples of the multi-modal colorization, and 
    \item Additional discussions on the limitations.
\end{itemize}

\section{Details on Network Architecture}
% 그림[]는 우리의 encoder-generator model의 overview를 나타낸다.
% 우리는 최적의 encoder-generator architecture를 찾고자 시도하였다. 
% 먼저 encoder의 설계를 위해, 우리는 다양한 activation function, ~를 search하였으며, which amount to BigGAN의 architecture와 유사한 형태로 ,other than Non local layer. 
% Non-local layer 빠진 이유
% Drop-out module 추가
% For generator, 우리는 BigGAN의 high level layer를 사용 (초기화)
% High level layer를 사용하기 때문에, 기존 BigGAN과 다르게 z의 dimension이 달라짐
\Fig{\ref{fig:sup_architecture_detail}} shows the detailed network architecture of {\MethodName}. %network overview of {\MethodName} and encoder-generator architecture in details. %.  \Fig{\ref{fig:sup_architecture_detail}}(b) and (c) show our encoder and generator architectures. 
%\Fig{\ref{fig:sup_architecture_detail}} shows an overview of our encoder-generator model, and \Fig{\ref{fig:sup_encoder}} and %\Fig{\ref{fig:sup_generator}} represent a ResBlock of encoder and generator, respectively.
We designed our encoder architecture by inverting the original BigGAN generator~\cite{BigGAN}. % with the following changes.
%Specifically, we conduct ablation studies of various layers in the BigGAN including activation functions, sequence of the modules, normalization scheme, non-local layer, and drop-out module. \sh{Did we show all the ablation results in the main paper?} \kkang{이 부분은 사실 architecture search 했다는 내용(어떻게 encoder 구조 만들지, layer는 어떻게 쌓고 activation function은 어떻게 사용할지..)이며 이 부분 역시 모두 encoder에 대한 내용입니다.} \kkw{이 부분에 대해서 첨부된 ablation 결과는 따로 없습니다.}
Specifically, our encoder consists of several ResBlocks, which is designed based on the ResBlock of the generator with a couple of modifications.
Specifically, while the generator of BigGAN has non-local layers in a few ResBlocks, we exclude them from the encoder, and we adopt an additional drop-out layer at the end of each ResBlock for performance improvement.
For the generator, we adopt the network architecture of the fine-scale layers of the BigGAN generator.
% Compared to the ResBlocks of the generator, the ResBlock of the encoder does not have non-local layers, but has an additional drop-out layer for performance improvement.
% Specifically, we exclude non-local layers and add drop-out layers for performance improvements.
% Our generator has the same design with the fine-scale layers of the BigGAN generator~\cite{BigGAN}.
%\kkang{교수님 이 부분은 encoder part에 대한 변경사항이며, generator part는 BigGAN generator와 동일합니다.}
%To find an optimal encoder architecture, we investigated the type of activation functions, sequence of the modules, and various normalization schemes, which amount to the current architecture analogous to the BigGAN~\cite{BigGAN} generator.
%The non-local layer, a crucial component of the original BigGAN generator, is excluded in our encoder due to no performance improvement experimentally.
%The drop-out module is included as it slightly improves the qualitative performance.
We initialize the generator with a pretrained BigGAN model on the ImageNet-1K training set~\cite{ImageNet}.
The random vector $z$ fed to the generator has a dimension of $68$, %$\mathbb{R}^{68\times1}$
which splits into four $17$-dim vectors. % of $\mathbb{R}^{17\times1}$. %unlike to $119$ dimensions of the latent vector of the original BigGAN generator. 
We concatenate each split vector with the class code $c$ of dimension $128$,
resulting in a $145$-dim vector. %\mathbb{R}^{128\times1}$, resulting in a vector of $\mathbb{R}^{145\times1}$ that is injected to the generator. 
%See \Fig{\ref{fig:sup_architecture_detail}}.
Our code will be made public upon the acceptance of the paper.

%The random-sampled $z$ is split into four vectors of $17$ dimension, and each vector is concatenated with class code $c$ amounting to $145 $ dimension.
\input{figures_supple/architecture_detail}
%\input{figures_supple/encoder}
%\input{figures_supple/generator}

% We attempted to find an optimal encoder architecture considering the type of activation functions, sequence of the modules, various normalization schemes.
% After thorough architecture search, we amount to the current encoder architecture, resulting in the architecture analogous to the BigGAN generator. 
% The non-local layer, an crucial component of the original BigGAN generator, is excluded in our encoder due to no performance improvement experimentally.
% Drop-out module slightly improve the qualitative performance.

% For the generator, we adopt fine layers of BigGAN initialized with pretrained parameters using ImageNet1K training set with $256 \times 256$ resolution. 
% The random-sampled $z$ has a dimension of $68 \times 1$, which is different from the original dimension of 119 x 1, as we only use part of the BigGAN generator.
% This one dimensional vector is divided into four parts of $17 \times 1$ resolution, concatenated with class code $c$ and amount to $145 \times 1$ dimension.
% See \Fig\ref{fig:sup_architecture_detail}.

\section{User Study}
We designed an Amazon-Mechanical-Turk interface for our user study as shown in \Fig{\ref{fig:sup_userstudy_gui}}. 
For an input grayscale image, a user should select the most preferred colorization image among the results with different methods.
In total, there are 100 test samples.
We shuffled the order of the results to remove any bias in the sequence. %color image results for all tests.
We also intentionally added the input grayscale image as a trap option in the colorization results for the sanity check of the user study.
%in order to collect experimental data from users who provided valid choices, 
%for the differennt results. The trap image is identical to the grayscale reference image. 
We excluded all the subjects who selected the trap image at least one time.
In this way, we selected 33 valid participants out of 200 total subjects. %, amounting to selected 33 participants.
\Tbl{\ref{table:sup_user_study_detail}} shows the full preference scores of all of the participants and statistics that summarize the user scores.
The results show that the participants generally prefer to the results of \MethodName~over the others.
%, demonstrating the effectiveness of {\MethodName}.

\section{Additional Assessment}
\subsection{Impact of Color Augmentation}
%Our color augmentation strategy slightly alters the colors of the real images in the training set
%Our color augmentation strategy enhances the vividness and semantic correctness of synthesized color images by making th
Our color augmentation strategy enhances the vividness and semantic correctness of synthesized color images by slightly altering the colors in the real images in the training set.
Specifically, our color augmentation strategy boosts the colors in the real images in the training set, which is fed to the discriminator during training, only by a small amount so that it does not introduce unwanted distortion to the color distribution of real images.
On the other hand, it still makes the colors of semantically different regions in the training images more distinguishable during the training phase.
In consequence, it helps the generator learn to synthesize semantically more correct and vivid colors.
In this section, we qualitatively demonstrate the effect of our color augmentation.
For the quantitative evaluation, we refer the readers to Tab.~5 in the main manuscript.

\Fig{\ref{fig:sup_aug_cmp}} shows a qualitative comparison of our color augmentation strategy with two baselines: \Method\ without our augmentation and \MethodName\ with post color processing.
For the post color processing, we apply the same color color-balancing method used in \MethodName\ directly to the output of the generator.
%Note that \MethodName\ applies the color-balancing method only to the real samples fed to the discriminator during the training phase.

The results of \MethodName\ without the color augmentation and with the post color processing (\Fig{\ref{fig:sup_aug_cmp}}(b) and (c)) have similar colors while the the results in (c) are slightly more vivid. This implies that our color augmentation scheme does not change the color distribution of the real images in the training set much.
Also, compared to our results in (d), the results without the color augmentation have less vivid and semantically inaccurate colors, e.g., the dull colors of the bricks and wood on the first and second rows, the red color on the accordion on the fourth row, and the red human face on the last row.
While the post processing slightly boosts the color vividness, its results still have the exactly same artifacts as it is applied at the end of the colorization process.
On the other hand, our results have more vivid and semantically correct colors, showing that our color augmentation scheme helps the generator synthesize more vivid and accurate colors.

% human face in the last row is colorized red by the other methods, while 
% As shown by the results of \MethodName\ with post color processing, our color augmentation scheme slightly alters the colors in input images

% We evaluate the impact of our color augmentation by showing a qualitative comparison. 
% See Tab. 5 of the main manuscript for quantitative evaluation.
% \Fig{\ref{fig:sup_aug_cmp}} shows that our color augmentation improves both naturalness and vividness of synthesized color images compared to two baselines: 
% \MethodName\ without our color augmentation and \MethodName\ with a post color processing. 
% For the post color processing, we apply the same color-balancing method used in \MethodName\ to the output of the generator.
% Note that \MethodName\ applies the color-balancing to the real samples fed to the discriminator. 
% Color augmentation of \MethodName\ enables natural and vivid colorization as shown in \Fig{\ref{fig:sup_aug_cmp}}, specifically the bricks, the wood texture, the dog, and the human faces.


\subsection{Luminance Replacement}
% fig : sup_rgb_lab
\MethodName\ brings the high-frequency spatial details of the input grayscale image via luminance replacement.
%exploit high-frequency details of input image by replacing the luminance of synthesized image with input luminance in the CIELAB color space.
\Fig{\ref{fig:sup_rgb_lab}} shows that the luminance replacement enables us to recover high-frequency spatial details while maintaining the high-quality colors synthesized from our generator. % compares the output of the generator and the result of replacing the luminance as described in \Fig{\ref{fig:ablation_fdim_teaser}} (d) and (e) in the main paper.
%Although the generator output also shows good colorization results, the image detail is greatly improved by replacing luminance.


%N
%Our color augmentation scheme enables not only enhancing vividness of color of each semantic part but also estimating more consistent and correct color, resulting in the better scores on FID~\cite{FID} and classification accuracy, as shown in Tab. 5. in the main paper.
%For instance, as shown in 1st and 2nd columns of \Fig{\ref{fig:sup_aug_cmp}}, our color augmentation scheme successfully enhance the colors of brick and wood textures.
%In addition, it helps to produce more consistent colors as shown in 3rd and 4th columns of \Fig{\ref{fig:sup_aug_cmp}}. While the leg guard of a dog is unnaturally colorized with two color even though it is single object in the case of the non-augmentation model, our full model produces a consistent color. 
%Lastly, it also helps to produce semantically accurate colors as shown in 5th and 6th of \Fig{\ref{fig:sup_aug_cmp}}.
%\kkw{Saturation Histogram 결과가 예상과 다름, trainging dataset에 대해서 시도 예정}


\section{Additional Comparisons}
%\section{Qualitative and Quantitative Comparison}
% 기존 방법 구현 details.
% 그림 설명
%\subsection{Implementation}
%In this section, we first describe the implementation details of the previous methods~\cite{TowardVivid,Deoldify,CIC,ChromaGAN,InstColor,ColTran} and then provide additional qualitative and quantitative comparisons. 
In this section, we provide additional qualitative and quantitative comparisons against recent colorization methods~\cite{TowardVivid,Deoldify,CIC,ChromaGAN,InstColor,ColTran}.
For the previous methods, we used the official codes from the authors except for ToVivid~\cite{TowardVivid}, which does not provide code at the time of our submission.
%We used the official codes for the previous methods except ToVivid~\cite{TowardVivid} which does not provide code at the time of our submission. 
For the results of ToVivid, we requested the authors, and obtained the results for our input images.
%Instead, the authors ToVivid~\cite{TowardVivid} directly provided results for our input images. %which we use directly. %Instead, we directly requested and received the results of ToVivid~\cite{TowardVivid} from the author.
We use the {\it stable} version of DeOldify~\cite{Deoldify}. % which shows better performance on the ImageNet~\cite{ImageNet} validation set.

As ColTran~\cite{ColTran} and ToVivid~\cite{TowardVivid} can only deal with images of a specific size, we conducted our experiments as follows.
For all the other methods except for ColTran and ToVivid, we resized the input images keeping the aspect ratio so that the smaller between the width and height is 256, performed colorization, and cropped the center regions.
Regarding ToVivid, we resized the input images to $256\times256$ ignoring the aspect ratio, obtained their colorization results, and resized the results to recover the original aspect ratios while keeping the smaller between the width and height is still 256. Then, we cropped the center regions of size $256\times256$.
Regarding ConTran, we resized the input images keeping the aspect ratio so that the smaller between the width and height is 256, cropped the center regions of size $256\times256$, and performed colorization.

% We evaluate state-of-the-art colorization methods for the images of resolution $256 \times 256$.
% This is because ColTran~\cite{ColTran} and ToVivid~\cite{TowardVivid} can only deal with the specified resolution. 
% \sh{check this paragraph:}
% %treat the fixed size input image with $256 \times 256$with For fair comparison, all colorized images should have identical spatial resolution. 
% %While the CNN-based colorization methods~\cite{CIC,ChromaGAN,InstColor,Deoldify} are free from the constraints to input resolution and aspect ratio, ColTran~\cite{ColTran} and ToVivid~\cite{TowardVivid} can only treat the fixed size input image with $256 \times 256$ due to their structure.
% To overcome this constraint, ToVivid~\cite{TowardVivid} adopted a trick that resizes the input image to $256 \times 256$ resolution ignoring the aspect ratio. ColTran~\cite{ColTran} resizes and center crops the input image to $256 \times 256$.
% Considering these aspects, in case of the CNN-based colorization methods and our methods, we center crop the colorization results according to ColTran~\cite{ColTran}, and in case of ToVivid~\cite{TowardVivid}, we restores the colorization results to the original aspect ratio and then center crops them.

\subsubsection{Qualitative Comparisons}
We show additional qualitative comparisons in \Fig{\ref{fig:sup_cmp1}}, \Fig{\ref{fig:sup_cmp2}}, and \Fig{\ref{fig:sup_cmp3}}. 
\MethodName\ outperforms all the compared methods for challenging scenes with diverse semantics and structures. % In these comparison, both images of complex structures and images of simple structures are included, and our method shows superior performance in both cases.

\subsubsection{Comparison on Challenging Images}
As described in the main manuscript, we constructed a curated dataset consisting of 100 complex images based on the number of people. %100 challenging image dataset by selecting images with complex structure based on the number of people.
\Fig{\ref{fig:sup_simple_vs_cplx}} shows representative examples of the simple images and complex images with respect to the number of people.
Note that the complex images not only contain many people, but also have higher image complexity.
%shows the thumbnails of the complex dataset and the whole dataset. Note that the curated complex dataset not only contains many people, but also has higher image complexity.  %of complex images compared to simple images. It can be seen that the challenging images not only includes a lot of people, but also images with a complex structure.
\Tbl{\ref{table:sup_cplx_fid_color}} and \Fig{\ref{fig:sup_cplx1}} show quantitative and qualitative comparisons of different colorization methods. 
Again, {\MethodName} achieves state-of-the-art quantitative and qualitative performance.
%FID~\cite{FID} and colorfulness score~\cite{Colorfulness}, and while the results of the previous methods show a big difference in quality for each input image, {\MethodName} easily produces vivid colorization results for all input images.

% For qualitative comparison to previous methods, we estimated the color results using official implementations for each method except for ToVivid~\cite{TowardVivid} due to the absence of released code.
% Instead of reproducing the method of ToVivid and directly estimating the color image from a grayscale image, we requested and received the colorization results of ToVivid~\cite{TowardVivid} from the author.
% For the case of DeOldify, which supports {\it stable} and {\it artistic} versions, we chose the stable version showing better performance on the ImageNet~\cite{ImageNet} validation set.

% For clear perceptual comparison, all estimated images require identical resolution.
% While the CNN-based colorization methods~\cite{CIC,ChromaGAN,InstColor,Deoldify} used in the comparison free from constraints to image resolution and aspect ratio, Coltran~\cite{ColTran} and ToVivid~\cite{TowardVivid} only enable producing the fixed size output with $256 \times 256$ spatial.
% To overcome the constraint, ToVivid adopted a trick that resizes the grayscale image to $256 \times 256$ resolution ignoring the aspect ratio.
% However, ColTran was vulnerable to the resizing trick due to their downsampling scheme of $64 \times 64$ low resolution.
% As a result, we used the $256 \times 256$ resolution for all qualitative comparisons to compare in a situation where all methods are operable.

% In this supplemental document, we provide more qualitative and quantitative comparisons. Specifically, qualitative comparison for general image in ImageNet1K validation set shown in \Figs{\ref{fig:sup_cmp1}~\ref{fig:sup_cmp2}~\ref{fig:sup_cmp3}}, qualitative and quantitative comparison for complex images shown in \Fig{\ref{fig:sup_cplx1}} and \Tbl{\ref{table:sup_cplx_fid_color}}.

\section{Additional Results}

\paragraph{Uncurated Examples}
\MethodName\ enables robust colorization for in-the-wild images. 
We show our colorization results on 100 \emph{uncurated} images in \Fig{\ref{fig:sup_uncurate1}} and \Fig{\ref{fig:sup_uncurate2}}.
%See \Fig{\ref{fig:sup_uncurate_cmp}} for the other compared methods that fail on the challenging uncurated scenes.

\subsection{Multi-modal Colorization}
\MethodName\ allows us to synthesize diverse colors for an input grayscale image.
\Fig{\ref{fig:sup_multimodal}} shows additional results of multi-modal colorization by using different random codes $z$. %, {\MethodName} colorize input the grayscale image with a different color that a given class would represent.

\subsection{Limitations}
% fig : sup_limitation
\Fig{\ref{fig:sup_limitation}} shows three failure cases of \MethodName.
First, {\MethodName} may fail to colorize very small regions such as the ear in the first row in the figure. This is because the spatial resolution of extracted feature $f$ is small as $16\times16$. %, meaning that small regions might be overlooked.
Second, {\MethodName} may struggle with complex images that contain objects with significantly different object classes such as toys and human. %In this example, the class of the image is the toy class, which contaminates the hand with toy color. 
%\kkang{추정되는 근본 원인: 이미지의 class는 장난감으로 붉은 색과 같은 color가 많이 포함됨. 이는 손과 같은  경계이면서 애매한 부분에 장난감 color를 칠해버리는 결과를 산출함, 즉 단일 class로 한 이미지가 정의되어서 생성되는 문제...}
Lastly, {\MethodName} may fail to handle input images considerably different from training images. 
%That is, input grayscale images are expected to lie in a similar distribution of training grayscale images.
Old grayscale photographs could fall into such category. Old photographs deviate from the training-data grayscale distribution due to its film sensitivity and chemical development recipes.
 %  with  input grayscale images often fail to estimate proper color on low quality grayscale images.
%This is because deterioration such as blur or noise of the low quality image deviates the image from the learned distribution of {\MethodName}.

% We provide more qualitative examples of BigColor, consisting of multi-modal solutions with random code $z$ shown in \Fig{\ref{fig:sup_multimodal}}, color results before and after Lab fusion shown in \Fig{\ref{fig:sup_rgb_lab}}, uncureated colorization results shown in \Figs{\ref{fig:sup_uncurate1}~\ref{fig:sup_uncurate2}}, and examples with limitations shown in \Fig{\ref{fig:sup_limitation}}.\kkw{Describe detail of limitation}

% As shown in \Fig\ref{fig:sup_userstudy_gui}, we use a trap image for all test samples in order to filter the insincere participants in Amazon Mechanical Turk (AMT). The trap image is identical to the grayscale reference image. We excluded the subjects who select the trap image as the best colorization result at least one of the 100 test samples. In this way, we found 167 unfaithful ones from 200 total subjects, amounting to selected 33 participants. To select the 100 grayscale images for the test, we randomly sampled color images from ImageNet1K validation set, applied the grayscale transformation, and estimated the color for gray inputs using target colorization methods. To avoid potential bias from the method order, we shuffled the sequence of color image results for all tests.

%%%%%%%%%%%%%%% TEXT END %%%%%%%%%%%%%%%

\input{figures_supple/userstudy_gui}
\input{tables_supple/tbl_userstudy}

\input{figures_supple/aug_cmp}
\input{figures_supple/rgb_lab}

\input{figures_supple/cmp}
\input{figures_supple/simple_vs_cplx}
\input{figures_supple/cplx}
\input{tables_supple/tbl_cplx_fid_color}

\input{figures_supple/uncurate}
\input{figures_supple/multimodal}
\input{figures_supple/limitation}
